Dictionary Learning from Incomplete Data

This paper extends the recently proposed and theoretically justified iterative thresholding and $K$ residual means algorithm ITKrM to learning dicionaries from incomplete/masked training data (ITKrMM). It further adapts the algorithm to the presence of a low rank component in the data and provides a strategy for recovering this low rank component again from incomplete data. Several synthetic experiments show the advantages of incorporating information about the corruption into the algorithm. Finally, image inpainting is considered as application example, which demonstrates the superior performance of ITKrMM in terms of speed at similar or better reconstruction quality compared to its closest dictionary learning counterpart.

==> sec_lr_old.tex <==
%%%%%%%%%%%%%%
%!TEX root = maskdl.tex

%%%%%%%%%%%
\section{Recovery of the lowrank component}\label{sec:lr}
%%%%%%%%%%%

%{\color{red} {\bf Responsible: Valeriya, updated : July 29}}
%
%{\it The main thing: sequential and parallelisable and computationally light! 
%Why don?t we do SVD: it is heavy, it is harder to incorporate the information on the mask. Refer to the robust PCA. 
%
%We would do something that is quite simple: one method is the power iteration for the SVD, incorporating the mask; the other version is an algorithm for dictionary learning with mask: ITKRM with $S=1$, which is equivalent to ITKSM with mask and every signal uses the same atom (no need to find $I_n$).
%Check references to l1-SVD (sparse PCA / robust PCA)?.
%
%Here the algorithm comes?. In the general version with the weight = $w(M_n y_n).$ Explain all parts of the algorithm + examples where this would be necessary + examples of several weights / updates. Refer to robust PCA again.}
%
%
%This we do by calculating the largest $\ell$ singular values with singular vectors of $\left(M_1y_1,\ldots ,M_N y_N\right)$.\\
%We need to prove that this can be done to arbitrary precision with high prob given $N(\ldots)$ signals.
%Later in the algorithm we always need to subtract the contribution of the low rank component $\tilde \dico_0 $
%and the contribution of the $S$ strongest atoms in the current guess of the dictionary.
%%%%%%%%%


%%%To identify the dictionary we first need to identify the low rank component.\\

Beyond the motivating applications in diabetes therapy management used in this paper, there are many important applications in which the data under study can naturally be modelled as a low-rank plus a sparse contribution. We mention, for instance, image, audio and video surveillance,  web search, etc. 
As mentioned earlier, without requiring the features/atoms to be orthogonal to the common low-rank component, one would likely obtain an ill-conditioned and coherent dictionary, where most atoms are distorted towards the low-rank component. Therefore, before identifying a dictionary, one needs to take care of the low-rank component. 
One approach discussed in \cite{ahelsa06} suggests to set a constant (non-zero) value in all entries of the first dictionary element, which takes part in all signal representations, whereas all other dictionary atoms remain with zero mean during all iterations. Another approach to handle the low-rank component could be to subtract the baseline or average signal from all the signals and then run the dictionary recovery on the modified signals. As can be seen, both these techniques provide an adaptation to the case when some dictionary atoms are used with probability 1 instead of $O(\sparsity/\natoms)$ for signal recovery.  
It might be tempting to apply one of the above mentioned techniques for the low-rank component identification. However, as mentioned in the previous section, in the case of the corrupted signals, when the action of the mask destroys the structure, we cannot assure that the masked dictionary will be orthogonal to the low-rank component, \ie, $\dico^\star M \lrcomp \neq 0$. Therefore, in this section we present an algorithm for recovering the low-rank component from corrupted signals. We start our discussion with a short survey of possible techniques for the low-rank component recovery and their properties. 

It is well-known fact that the optimal low-rank approximation can be straightforwardly obtained by computing the full Singular Value Decomposition (SVD) and then truncating it by selecting the top dominant singular values and their corresponding singular vectors. 
Unfortunately, for high-dimensional large data sets the computation of the full SVD is numerically infeasible: computationally costly and memory intensive. Simultaneously with the computational prohibitiveness of the full SVD that can be partially overcome by utilising recently developed memory-efficient methods for randomised SVD \cite{hamatr11}, another major shortcoming of the SVD is its fragility with respect to highly corrupted and/or incomplete data, which is the prime focus of the current paper.  
%we need to address another challenge of the low-rank component approximation from incomplete data. 
One can argue that the latter problem, also known in the community as low-rank matrix completion problem,  can be solved by employing the recently developed Robust PCA \cite{calimawr11}, for instance. 
Despite its satisfactory performance and a number of optimality properties, our framework is slightly different, which do not allow us to employ techniques for the matrix completion problem in a straightforward way. In particular, differently to the Robust PCA, the mask provide us with the information on the location of the corruptions, which could be and should be incorporated in the recovery algorithm.  At the same time, we drop the assumption that the signal's observed entries are uniformly distributed among all sets, as exemplified with numerical experiments in Section 5.
%Finally, as we explain in the next section, our corrupted signal even after the extraction of the low-rank component cannot be assumed to be sparse in the generating dictionary $\dico$ but in its corrupted version $M \dico$. 

Ideally, we would like to use an easy and fast algorithm allowing for sequential low-rank component recovery. The latter could be quite beneficial if the rank $L$ of the low-rank component is unknown and the algorithm should adaptively identify it. It could be appealing to employ the power iteration method for the SVD \cite{mipo29}, which approximates singular values one-by-one. Whereas the method is simple and fast in special cases with uncorrupted data, incorporation of the mask into singular value recovery is again expected to be quite tedious. In addition, once the corruption pattern is not homogenous, the adjustment and usage of the method is expected to be quite tricky. Another quite natural alternative for the recovery of the low-rank component is to employ a modified version of the earlier presented ITKrMM algorithm.
%%%
%For the sake of concise and simple presentation, we assume that the rank of the low-rank component is one, i.e., $\rank(\lrcomp) = 1.$ However, as noted earlier the idea is that the algorithm recovers low-rank component in the subsequent fashion, i.e., $\sum_{r=1}^{\rank(\lrcomp)} \lratom_i.$ 

For the sake of concise and simple presentation of the algorithm, it will be enough to discuss the simplest case where the low-rank coefficient is with equal probability $\pm \scale_\lrc$ for $\scale_\lrc \gg \sqrt{S}/K$, the coefficient sequence $c$ has the shape $c(k)=1/\sqrt{S}$ for $k\leq S$ and $c(k) =0$ for $k>S$ .\\

The algorithm for the low-rank component recovery is essentially a modified version of the ITKrMM algorithm, which during each call recovers only one element of the low-rank component, \ie, $\lrcomp = (\lratom)$ by performing the atom update as normalised signed mean of all training signals. Since the low-rank component is expected to be present in (mostly) all signals, we can omit step 1 in the ITKrMM algorithm related to the support recovery by the thresholding.  
Due the structure of the algorithm, the atom update - normalised signed mean of the training signals - is performed by processing one signal at a time. 

%{\bf Text below to be modified in line with Section 3.

%The ITKrM algorithm for the low-rank component recovery is essentially a modified version of the $K-$means algorithm, which solves the following maximisation problem
%\[
 %\max_{\lrcomp \in D} \sum_n \max_i |\langle y_n, \lratom_i \rangle|
%\]
%for a family of given signals $y_n.$ The $K-$means algorithm is an iterative method, which in each iteration assigns each training signal to the atom of the current dictionary giving the largest response in absolute value and then updating the atom as normalised signed mean of the associated training signals.}

%The low-rank recovery problem from corrupted data can be viewed as modification of the $K-$means algorithm, where our signal model is given as $My = M\lrcomp \lrc + M\dico_{I} x(I).$  Contrary to the classical $K-$means,  our algorithm  during each call recovers only one element of the low-rank component, \ie, $\lrcomp = (\lratom),$ and, thus, 
%only one step related to the atom update needs to be performed.  

%Due the structure of the algorithm, the atom update - normalised signed mean of the
%training signals - is performed by processing one signal at a time. 

%Note that due to the nature of the signals,  we need to ensure that the recovered component is orthogonal to the generating dictionary by providing a proper dictionary representation of the corrupted signal. To be more precise, we account for the variance in the norm of the corrupted atom by introducing the factor $\frac{1}{{\|M_n \lratom\|_2}}$ in the update of $\bar \lratom.$ 
%On the contrary to the well-recognised Robust PCA and similar methods, we do not assume that the corruptions are uniformly distributed inside and across the signals. 
%A simple and quite intuitive recipe to deal with such situation is to introduce a weight function $\omega(M_n)$ into the updates. It will allow to compensate correctly for the presence of highly corrupted or vice versa completely clean signals. 
As also for the dictionary learning part, presented in Section 3, we need to ensure that the recovered component is orthogonal to the generating dictionary by accounting for the variance in the norm of the corrupted atom $\frac{1}{{\|M_n \lratom\|_2}}.$ However, this factor appears only under the $\signop$ function and we recall that $\signop(\ip{M_n \lratom }{M_n y_n}/\|M_n \lratom\|_2) =\signop(\ip{\lratom}{M_n y_n})$.

Once all signals are processed, the update is done by rescaling the atom according to the number of observations and removing any possible contribution of the previously recovered low-rank component (relevant only for the case $L>1$) by projecting the new atom into the reconstructed low-rank component and then performing the normalisation step. 
Note also that for the case $L>1,$ before turning into the recovery of the subsequent component, one  should ensure that the contribution of the already recovered low-rank component has been removed from the data. This is done by projecting the data onto the corrupted low-rank component.

%%%% LR Component Algorithm
\begin{algorithm}[ITKrMM for the low-rank component recovery with corrupted data -  one iteration for one low-rank component] 

Given previously recovered low-rank components $\lrcomp = (\lratom_i),$ an input low-rank component $\tilde \lrcomp = (\tilde \lratom),$ and $\tilde N$ corrupted training signals $y^M_n=(M_ny_n,M_n)$ do:\\

For all $n$
\begin{itemize}
\item Subtract contribution of the previously recovered low-rank component $\Gamma$ from the data $\bar  y_n = Q(M_n \Gamma) M_n y_n,$
%find $I_n^t= \arg\max_{I: |I| = S}  \sum_{i\in I: M_n \atom_i \neq 0} \frac{| \ip{M_n \atom_i}{y_n}|}{\|M_n \atom_i\|_2}$.
\item Calculate
\[
%\bar \lratom = \frac{1}{\tilde N} \sum_{n} M_n \bar y_n \signop (\langle  M_n \bar  y_n, \tilde \lratom \rangle ) \quad \mbox{ and } \quad  W = \| M_n \|_1
\bar \lratom = \frac{1}{\tilde N} \sum_{n} (\I_d - P(M_n \lrcomp) + P(M_n \tilde \lratom_n) ) M_n y_n\signop (\langle  M_n \bar  y_n, \tilde \lratom_n \rangle ) \quad \mbox{ and } \quad  W = \| M_n \|_1
\]
% \frac{|\langle  y_n, M_n \tilde \lratom \rangle |}{ \|M_n \tilde \lratom\|_2 }  \cdot \omega(M_n).
%\sum_{n: k\in I_n^t} \big[\I_d - P(M_n(\tilde \lrcomp,\pdico_{I_n^t})) + P(M_n \patom_k)\big] M_n  y_n \cdot \signop(\ip{\patom_k}{M_n y_n})  \\
%\mbox{ and }\qquad W= \frac{1}{d} \| M_n \|_{1}.
%\patomn_k= \sum_{n: k\in I_{n}^t} \big[\I - P&(\pdico_{I_{n}^t})  + P(\patom_k) \big] y_n \cdot \signop(\ip{\patom_k}{y_n}),\notag %\cdot  \chi(I_n^t, k),

\item Set $\bar \plratom = Q(\Gamma) W^{-1} \plratom$ and output $\bar \plrcomp = (\bar \plratom / \| \bar \plratom \|_2)$.
%\item Ensure that  $\dico^\star \tilde \lrcomp = 0$.
\end{itemize}

\end{algorithm}

Similarly to ITKrMM, this algorithm can be stopped after a fixed number of iterations or once a stopping criteria is reached. As reported in \cite{sc15b} the algorithm has very low computational complexity and with a high probability the algorithm converges locally to the generating dictionary. 

%We should note that for $L>1,$ \ie, when the rank of the low-rank component is larger than 1,  the above algorithm does not need to be modified. However, before turning into the recovery of the subsequent components, one  should ensure that the contribution of the already recovered low-rank component has been removed by projecting the data into the corrupted low-rank component, \ie,
%\[
%M_n \bar  y_n = M_n y_n - P(\bar \lrcomp) M_n y_n,
%\]
%and using these signals as new inputs to the ITKrM algorithm. Eventually, we need to remove any possible contribution of the previously recovered low-rank component from the subsequent ones by again projecting the new atom into the reconstructed low-rank component and then performing the normalisation step. 

